N-Gram Graph: Simple Unsupervised Representation for Graphs, with Applications to Molecules

Machine learning techniques have recently been adopted in various applications in medicine, biology, chemistry, and material engineering. An important task is to predict the properties of molecules, which serves as the main subroutine in many downstream applications such as virtual screening and drug design. Despite the increasing interest, the key challenge is to construct proper representations of molecules for learning algorithms. This paper introduces the N-gram graph, a simple unsupervised representation for molecules. The method first embeds the vertices in the molecule graph. It then constructs a compact representation for the graph by assembling the vertex embeddings in short walks in the graph, which we show is equivalent to a simple graph neural network that needs no training. The representations can thus be efficiently computed and then used with supervised learning methods for prediction. Experiments on 60 tasks from 10 benchmark datasets demonstrate its advantages over both popular graph neural networks and traditional representation methods. This is complemented by theoretical analysis showing its strong representation and prediction power.

==> table/effect_of_N_R_regression.tex <==

\begin{table}[H]
    \centering
    \caption{Root mean squared error (RMSE) on three regression tasks with different combinations of $r$ and $n$.
             In task Malaria and CEP, we can observe that when using XGBoost (XGB) and Random Forest (RF), in the most cases, the RMSE will get smaller with larger N-gram dimension $N$ and larger projection dimension $r$.
             This can be explained that with larger $N$ and larger $r$, N-gram can contain more information, and the training will be more accurate.
             However, this doesn't hold on task Delaney, where the RMSE fluctuates a lot.
             }
    \begin{tabular}{|c|c|c|c|c|}
\hline
target name	&$r$-dim	&$n$-gram	&RF	&XGB	\\
\hline\hline
\multirowcell{6}{Delaney}	&\multirow{3}{*}{50}	&2	&	0.787 $\pm$ 0.019	&	\textbf{0.751 $\pm$ 0.034}	\\
\cline{3-5}
	&	&4	&	0.818 $\pm$ 0.018	&	\textbf{0.745 $\pm$ 0.015}	\\
\cline{3-5}
	&	&6	&	0.831 $\pm$ 0.019	&	\textbf{0.766 $\pm$ 0.026}	\\
\cline{2-5}
	&\multirow{3}{*}{100}	&2	&	0.831 $\pm$ 0.025	&	\textbf{0.737 $\pm$ 0.024}	\\
\cline{3-5}
	&	&4	&	0.874 $\pm$ 0.027	&	\textbf{0.756 $\pm$ 0.045}	\\
\cline{3-5}
	&	&6	&	0.893 $\pm$ 0.029	&	\textbf{0.782 $\pm$ 0.045}	\\
\hline
\multirowcell{6}{Malaria}	&\multirow{3}{*}{50}	&2	&	1.051 $\pm$ 0.017	&	\textbf{1.050 $\pm$ 0.014}	\\
\cline{3-5}
	&	&4	&	1.034 $\pm$ 0.017	&	\textbf{1.032 $\pm$ 0.014}	\\
\cline{3-5}
	&	&6	&	1.031 $\pm$ 0.016	&	\textbf{1.028 $\pm$ 0.016}	\\
\cline{2-5}
	&\multirow{3}{*}{100}	&2	&	\textbf{1.050 $\pm$ 0.014}	&	1.061 $\pm$ 0.017	\\
\cline{3-5}
	&	&4	&	1.029 $\pm$ 0.013	&	\textbf{1.022 $\pm$ 0.014}	\\
\cline{3-5}
	&	&6	&	1.027 $\pm$ 0.013	&	\textbf{1.019 $\pm$ 0.012}	\\
\hline
\multirowcell{6}{CEP}	&\multirow{3}{*}{50}	&2	&	1.497 $\pm$ 0.010	&	\textbf{1.457 $\pm$ 0.013}	\\
\cline{3-5}
	&	&4	&	1.458 $\pm$ 0.008	&	\textbf{1.373 $\pm$ 0.011}	\\
\cline{3-5}
	&	&6	&	1.458 $\pm$ 0.007	&	\textbf{1.339 $\pm$ 0.011}	\\
\cline{2-5}
	&\multirow{3}{*}{100}	&2	&	1.533 $\pm$ 0.008	&	\textbf{1.485 $\pm$ 0.010}	\\
\cline{3-5}
	&	&4	&	1.533 $\pm$ 0.004	&	\textbf{1.391 $\pm$ 0.015}	\\
\cline{3-5}
	&	&6	&	1.545 $\pm$ 0.005	&	\textbf{1.373 $\pm$ 0.005}	\\
\hline
    \end{tabular}
    \label{tab:n_gram_regression}
\end{table}

==> table/effect_of_N_R_tox21.tex <==

\begin{center}
    \begin{longtable}{|c|c|c|c|c|}
    \caption{This table includes Random Forest (RF) and XGBoost (XGB) on N-gram graph.
             Two values for $r$ and three values for $N$ are tested.
             For each combination, model with best performance is \textbf{bolded}.
             For most of the cases, XGB has larger ROC than RF, and larger n-gram number $N$ usually leads to better performance.
             And on the random projection dimension $r$, larger $r$ does not show an obvious improvement.
             }
    \label{tab:tox21_complete_n_gram}
    \endfirsthead
    \endhead
\hline
target name	&$r$-dimension	&$n$-gram	&RF	&XGBoost	\\
\hline\hline
\multirow{5}{*}{NR-AR}	&\multirow{3}{*}{50}	&2	&	\textbf{0.803 $\pm$ 0.032}	&	0.799 $\pm$ 0.037	\\
\cline{3-5}
	&	&4	&	\textbf{0.801 $\pm$ 0.039}	&	0.790 $\pm$ 0.042	\\
\cline{3-5}
	&	&6	&	\textbf{0.798 $\pm$ 0.034}	&	0.797 $\pm$ 0.033	\\
\cline{2-5}
	&\multirow{3}{*}{100}	&2	&	\textbf{0.803 $\pm$ 0.037}	&	0.798 $\pm$ 0.040	\\
\cline{3-5}
	&	&4	&	\textbf{0.800 $\pm$ 0.039}	&	0.788 $\pm$ 0.037	\\
\cline{3-5}
	&	&6	&	0.801 $\pm$ 0.036	&	\textbf{0.801 $\pm$ 0.037}	\\
\cline{1-5}
\multirow{5}{*}{NR-AR-LBD}	&\multirow{3}{*}{50}	&2	&	\textbf{0.857 $\pm$ 0.016}	&	0.854 $\pm$ 0.013	\\
\cline{3-5}
	&	&4	&	\textbf{0.859 $\pm$ 0.025}	&	0.848 $\pm$ 0.018	\\
\cline{3-5}
	&	&6	&	\textbf{0.862 $\pm$ 0.023}	&	0.854 $\pm$ 0.023	\\
\cline{2-5}
	&\multirow{3}{*}{100}	&2	&	0.855 $\pm$ 0.013	&	\textbf{0.864 $\pm$ 0.013}	\\
\cline{3-5}
	&	&4	&	0.856 $\pm$ 0.011	&	\textbf{0.866 $\pm$ 0.017}	\\
\cline{3-5}
	&	&6	&	\textbf{0.863 $\pm$ 0.015}	&	0.862 $\pm$ 0.012	\\
\cline{1-5}
\multirow{5}{*}{NR-AhR}	&\multirow{3}{*}{50}	&2	&	0.891 $\pm$ 0.008	&	\textbf{0.897 $\pm$ 0.009}	\\
\cline{3-5}
	&	&4	&	0.893 $\pm$ 0.008	&	\textbf{0.899 $\pm$ 0.011}	\\
\cline{3-5}
	&	&6	&	0.893 $\pm$ 0.008	&	\textbf{0.900 $\pm$ 0.011}	\\
\cline{2-5}
	&\multirow{3}{*}{100}	&2	&	0.883 $\pm$ 0.009	&	\textbf{0.890 $\pm$ 0.009}	\\
\cline{3-5}
	&	&4	&	0.888 $\pm$ 0.011	&	\textbf{0.894 $\pm$ 0.010}	\\
\cline{3-5}
	&	&6	&	0.888 $\pm$ 0.010	&	\textbf{0.895 $\pm$ 0.011}	\\
\cline{1-5}
\multirow{5}{*}{NR-Aromatase}	&\multirow{3}{*}{50}	&2	&	\textbf{0.845 $\pm$ 0.036}	&	0.842 $\pm$ 0.024	\\
\cline{3-5}
	&	&4	&	\textbf{0.852 $\pm$ 0.038}	&	0.850 $\pm$ 0.028	\\
\cline{3-5}
	&	&6	&	\textbf{0.853 $\pm$ 0.038}	&	0.851 $\pm$ 0.030	\\
\cline{2-5}
	&\multirow{3}{*}{100}	&2	&	0.843 $\pm$ 0.038	&	\textbf{0.851 $\pm$ 0.024}	\\
\cline{3-5}
	&	&4	&	0.847 $\pm$ 0.038	&	\textbf{0.855 $\pm$ 0.027}	\\
\cline{3-5}
	&	&6	&	0.847 $\pm$ 0.038	&	\textbf{0.853 $\pm$ 0.024}	\\
\cline{1-5}
\multirow{5}{*}{NR-ER}	&\multirow{3}{*}{50}	&2	&	\textbf{0.727 $\pm$ 0.015}	&	0.723 $\pm$ 0.024	\\
\cline{3-5}
	&	&4	&	\textbf{0.726 $\pm$ 0.016}	&	0.724 $\pm$ 0.012	\\
\cline{3-5}
	&	&6	&	0.730 $\pm$ 0.016	&	\textbf{0.732 $\pm$ 0.015}	\\
\cline{2-5}
	&\multirow{3}{*}{100}	&2	&	0.727 $\pm$ 0.019	&	\textbf{0.736 $\pm$ 0.016}	\\
\cline{3-5}
	&	&4	&	0.733 $\pm$ 0.020	&	\textbf{0.742 $\pm$ 0.012}	\\
\cline{3-5}
	&	&6	&	0.733 $\pm$ 0.022	&	\textbf{0.744 $\pm$ 0.014}	\\
\cline{1-5}
\multirow{5}{*}{NR-ER-LBD}	&\multirow{3}{*}{50}	&2	&	0.815 $\pm$ 0.021	&	\textbf{0.822 $\pm$ 0.012}	\\
\cline{3-5}
	&	&4	&	\textbf{0.820 $\pm$ 0.018}	&	0.813 $\pm$ 0.010	\\
\cline{3-5}
	&	&6	&	0.818 $\pm$ 0.018	&	\textbf{0.829 $\pm$ 0.014}	\\
\cline{2-5}
	&\multirow{3}{*}{100}	&2	&	0.819 $\pm$ 0.019	&	\textbf{0.830 $\pm$ 0.013}	\\
\cline{3-5}
	&	&4	&	0.826 $\pm$ 0.024	&	\textbf{0.832 $\pm$ 0.014}	\\
\cline{3-5}
	&	&6	&	0.825 $\pm$ 0.024	&	\textbf{0.830 $\pm$ 0.021}	\\
\cline{1-5}
\newpage
\hline
\multirow{5}{*}{NR-PPAR-gamma}	&\multirow{3}{*}{50}	&2	&	\textbf{0.832 $\pm$ 0.042}	&	0.811 $\pm$ 0.035	\\
\cline{3-5}
	&	&4	&	\textbf{0.834 $\pm$ 0.042}	&	0.825 $\pm$ 0.043	\\
\cline{3-5}
	&	&6	&	\textbf{0.836 $\pm$ 0.040}	&	0.826 $\pm$ 0.043	\\
\cline{2-5}
	&\multirow{3}{*}{100}	&2	&	0.834 $\pm$ 0.030	&	\textbf{0.840 $\pm$ 0.032}	\\
\cline{3-5}
	&	&4	&	\textbf{0.839 $\pm$ 0.031}	&	0.837 $\pm$ 0.032	\\
\cline{3-5}
	&	&6	&	0.835 $\pm$ 0.030	&	\textbf{0.835 $\pm$ 0.025}	\\
\cline{1-5}
\multirow{5}{*}{SR-ARE}	&\multirow{3}{*}{50}	&2	&	0.817 $\pm$ 0.012	&	\textbf{0.823 $\pm$ 0.013}	\\
\cline{3-5}
	&	&4	&	0.825 $\pm$ 0.014	&	\textbf{0.833 $\pm$ 0.012}	\\
\cline{3-5}
	&	&6	&	0.821 $\pm$ 0.016	&	\textbf{0.831 $\pm$ 0.014}	\\
\cline{2-5}
	&\multirow{3}{*}{100}	&2	&	0.824 $\pm$ 0.016	&	\textbf{0.833 $\pm$ 0.020}	\\
\cline{3-5}
	&	&4	&	0.828 $\pm$ 0.017	&	\textbf{0.838 $\pm$ 0.014}	\\
\cline{3-5}
	&	&6	&	0.827 $\pm$ 0.017	&	\textbf{0.833 $\pm$ 0.014}	\\
\cline{1-5}
\multirow{5}{*}{SR-ATAD5}	&\multirow{3}{*}{50}	&2	&	0.849 $\pm$ 0.010	&	\textbf{0.854 $\pm$ 0.009}	\\
\cline{3-5}
	&	&4	&	0.859 $\pm$ 0.013	&	\textbf{0.861 $\pm$ 0.016}	\\
\cline{3-5}
	&	&6	&	0.858 $\pm$ 0.011	&	\textbf{0.860 $\pm$ 0.011}	\\
\cline{2-5}
	&\multirow{3}{*}{100}	&2	&	0.835 $\pm$ 0.012	&	\textbf{0.848 $\pm$ 0.016}	\\
\cline{3-5}
	&	&4	&	0.854 $\pm$ 0.020	&	\textbf{0.857 $\pm$ 0.017}	\\
\cline{3-5}
	&	&6	&	0.851 $\pm$ 0.018	&	\textbf{0.852 $\pm$ 0.010}	\\
\cline{1-5}
\multirow{5}{*}{SR-HSE}	&\multirow{3}{*}{50}	&2	&	0.786 $\pm$ 0.023	&	\textbf{0.806 $\pm$ 0.025}	\\
\cline{3-5}
	&	&4	&	0.795 $\pm$ 0.027	&	\textbf{0.802 $\pm$ 0.022}	\\
\cline{3-5}
	&	&6	&	0.795 $\pm$ 0.025	&	\textbf{0.803 $\pm$ 0.022}	\\
\cline{2-5}
	&\multirow{3}{*}{100}	&2	&	0.781 $\pm$ 0.027	&	\textbf{0.783 $\pm$ 0.030}	\\
\cline{3-5}
	&	&4	&	\textbf{0.793 $\pm$ 0.020}	&	0.790 $\pm$ 0.026	\\
\cline{3-5}
	&	&6	&	0.791 $\pm$ 0.019	&	\textbf{0.793 $\pm$ 0.026}	\\
\cline{1-5}
\multirow{5}{*}{SR-MMP}	&\multirow{3}{*}{50}	&2	&	0.899 $\pm$ 0.008	&	\textbf{0.905 $\pm$ 0.007}	\\
\cline{3-5}
	&	&4	&	0.901 $\pm$ 0.011	&	\textbf{0.904 $\pm$ 0.013}	\\
\cline{3-5}
	&	&6	&	0.898 $\pm$ 0.010	&	\textbf{0.903 $\pm$ 0.015}	\\
\cline{2-5}
	&\multirow{3}{*}{100}	&2	&	0.900 $\pm$ 0.005	&	\textbf{0.907 $\pm$ 0.005}	\\
\cline{3-5}
	&	&4	&	0.903 $\pm$ 0.007	&	\textbf{0.910 $\pm$ 0.007}	\\
\cline{3-5}
	&	&6	&	0.902 $\pm$ 0.008	&	\textbf{0.908 $\pm$ 0.007}	\\
\cline{1-5}
\multirow{5}{*}{SR-p53}	&\multirow{3}{*}{50}	&2	&	0.844 $\pm$ 0.020	&	\textbf{0.852 $\pm$ 0.028}	\\
\cline{3-5}
	&	&4	&	0.844 $\pm$ 0.023	&	\textbf{0.853 $\pm$ 0.021}	\\
\cline{3-5}
	&	&6	&	0.842 $\pm$ 0.021	&	\textbf{0.848 $\pm$ 0.020}	\\
\cline{2-5}
	&\multirow{3}{*}{100}	&2	&	0.836 $\pm$ 0.013	&	\textbf{0.842 $\pm$ 0.021}	\\
\cline{3-5}
	&	&4	&	0.838 $\pm$ 0.015	&	\textbf{0.846 $\pm$ 0.024}	\\
\cline{3-5}
	&	&6	&	0.835 $\pm$ 0.014	&	\textbf{0.844 $\pm$ 0.020}	\\
\cline{1-5}
\multirow{5}{*}{Average}	&\multirow{3}{*}{50}	&2	&	0.831 $\pm$ 0.020	&	\textbf{0.832 $\pm$ 0.020}	\\
\cline{3-5}
	&	&4	&	\textbf{0.834 $\pm$ 0.023}	&	0.833 $\pm$ 0.021	\\
\cline{3-5}
	&	&6	&	0.834 $\pm$ 0.022	&	\textbf{0.836 $\pm$ 0.021}	\\
\cline{2-5}
	&\multirow{3}{*}{100}	&2	&	0.828 $\pm$ 0.020	&	\textbf{0.835 $\pm$ 0.020}	\\
\cline{3-5}
	&	&4	&	0.834 $\pm$ 0.021	&	\textbf{0.838 $\pm$ 0.020}	\\
\cline{3-5}
	&	&6	&	0.833 $\pm$ 0.021	&	\textbf{0.838 $\pm$ 0.018}	\\
\cline{1-5}
    \end{longtable}
\end{center}
